Coded Multi-User Information Retrieval with a Multi-Antenna Helper Node

A novel coding design is proposed to enhance information retrieval in a wireless network of users with partial access to the data, in the sense of observation, measurement, computation, or storage. Information exchange in the network is assisted by a multi-antenna base station (BS), with no direct access to the data. Accordingly, the missing parts of data are exchanged among users through an uplink (UL) step followed by a downlink (DL) step. In this paper, new coding strategies, inspired by coded caching (CC) techniques, are devised to enhance both UL and DL steps. In the UL step, users transmit encoded and properly combined parts of their accessible data to the BS. Then, during the DL step, the BS carries out the required processing on its received signals and forwards a proper combination of the resulting signal terms back to the users, enabling each user to retrieve the desired information. Using the devised coded data retrieval strategy, the data exchange in both UL and DL steps requires the same communication delay, measured by normalized delivery time (NDT). Furthermore, the NDT of the UL/DL step is shown to coincide with the optimal NDT of the original DL multi-input single-output CC scheme, in which the BS is connected to a centralized data library.

==> Intro-Old.tex <==
Multi-user information retrieval (MIR) is a generic field of research that explores proper mechanisms enabling each user to recover specific pieces of information that are either aggregated at a central master node or distributed across the network. The coded caching (CC) model is a promising approach to address the MIR problem in networks with centralized and distributed data. CC scheme has been originally proposed as a promising solution to reduce load during peak traffic times by employing the caches distributed in the network as a supplementary communication resource~\cite{maddah2014fundamental}. In a single-stream downlink network, the incorporation of CC boosts the achievable rate by a multiplicative factor that scales with the cumulative cache size in the entire network. This is accomplished by multicasting carefully designed codewords to a diverse set of users. In this context, implementing CC in a network serving $K$ users, each possessing sufficient memory to store a fraction $\gamma$ of the entire library, enables the so-called \emph{global coded caching gain} of $K\gamma+1$. Notably, this delivery speed-up factor can also be aggregated with the spatial multiplexing gain and enhanced to $K\gamma+L$ in a multi-input multi-output (MISO) setup with $L$ antennas at the transmitter~\cite{shariatpanahi2016multi,shariatpanahi2018physical}. The multi-user information retrieval problem in CC networks with centralized data at the BS has been studied in various models such as data shuffling~\cite{8957508,8955811,8754795}, private coded caching~\cite{9249022}, and cache-aided linear function retrieval~\cite{9378566,9681716}.

CC schemes can also be used to address the MIR problem in distributed computing systems. Distributed computing offers various advantages over centralized computing, such as enhanced scalability, reliability, and cost-effectiveness~\cite{book1}. Moreover, in many real-world applications~\cite{9463425}, including telecommunication networks (e.g., wireless sensor networks), time-sensitive process control (e.g., aircraft monitoring systems), and parallel computation (e.g., computer graphics), the data cannot be centrally aggregated due to the organizational or technical constraints, and the data recovery is carried out through the use of a cluster of devices working collaboratively. 
% These scenarios with distributed data share a common feature- they all operate as a CC model in which the base station (BS) is not directly linked to the library while the data is only partially available to the users.
For instance, the wireless MapReduce coded computing models are comprised of three phases: 1) Map Phase,  2) Shuffle phase, and 3) Reduce phase. During the Map phase, first, data is split and processed at distributed nodes, and in the shuffle phase, users transmit the results to a central server to complete the final process in the Reduce phase. This coded computing setup can be treated as a CC model in which, during the content placement phase, the system completes the Map tasks, and in the content delivery phase, it completes the Shuffle and Reduce phases in two consecutive steps.   


%The critical role of multi-antenna connectivity in resolving the practical bottlenecks of CC models has been explored in various studies. For instance, the authors in~\cite{lampiris2018adding,salehi2020lowcomplexity,parrinello2019fundamental} demonstrated the capability of MISO networks in reducing the subpacketization complexity in CC schemes. Moreover, in~\cite{10206827}, it was shown that employing the shared-cache model introduced in~\cite{parrinello2019fundamental} and equipping the transmitter with $L$ transmit antennas can effectively handle the CC configurations with the dynamic user population. The ability of MISO CC schemes to handle the media delivery in large-scale video-on-demand (VoD) and extended-reality (XR) applications has been studied in~\cite{9361706,salehi2022enhancing,mahmoodi2021non}. In addition, several works, including~\cite{tolli2017multi,8374074,9923619,10325409}, illustrated the enhancement in rate performance for MISO systems through the implementation of CC under finite signal-to-noise ratio (SNR) conditions. The multi-user information retrieval problem in CC networks with centralized data at the BS has been studied in various models such as data shuffling~\cite{8957508,8955811,8754795}, private coded caching~\cite{9249022}, and cache-aided linear function retrieval~\cite{9378566,9681716}.

   



% \todo[inline]{
% In this paper, we design novel coded techniques, inspired by coded caching (CC), to enhance data retrieval and distribution with the help of a central, multi-antenna transmit-receive point (TRP).

% This paper proposes novel coding techniques to enhance the performance of data retrieval and distribution in multi-user networks. Multi-user data retrieval and distribution is a key requirement of many emerging use cases. For example, (EXAMPLE OF VERTICAL OR SENSOR NETWORK). As another example, (EXAMPLE OF CODED COMPUTING OR BLOCKCHAIN). These examples clarify the importance of improving the efficiency of data retrieval and distribution using novel solutions. In this regard, we propose coding mechanisms inspired by the well-known coded caching (CC) technique that enhance data retrieval and distribution in multi-user networks with the help of a central base station (BS).

% The CC technique, proposed by ...

% The global caching gain of CC scales with the cumulative cache size of users and is additive with the spatial multiplexing gain of MISO and MIMO setups.

% Due to these nice properties, solving the practical bottlenecks of CC is considered by many papers. For example, (SUBPACKETIZATION), (FINITE-SNR), (DYNAMIC). On the other hand, other works have demonstrated the effectiveness of CC in handling media delivery in large-scale VoD (BAYAT,CAIRE) and XR (NARIMAN,OJCOMS) applications.

% The CC technique, however, was originally limited by definition to use cases where the content was cacheable in nature ... However, the underlying coding design of CC is indeed applicable to more diverse use cases. A prominent example is in distributed computing, where ... The original work on coded computing is later extended in a few notable directions, such as ...

% In this paper, we discuss how the coding design of CC can also be used to enhance general data retrieval and distribution in multi-user networks. (A SMALL DESCRIPTION OF SYSTEM MODEL). With a single-antenna BS, this problem is, in fact, similar to the well-studied two-way relaying networks (CITE). However, with a multi-antenna BS, using coded ...

% DISCUSSION ON THE CONTRIBUTION OF PAPER.
% }

 % The growing demand for emerging multimedia applications, such as video-on-demand (VoD) and extended reality (XR), consistently increases network congestion~\cite{cisco2018ciscob,salehi2022enhancing}. Coded caching (CC) has been proposed as a promising solution to reduce load during peak traffic times by employing the caches distributed in the network as a supplementary communication resource~\cite{maddah2014fundamental}. In a single-stream downlink network, the incorporation of CC boosts the achievable rate by a multiplicative factor that scales with the cumulative cache size in the entire network. This is accomplished by multicasting carefully designed codewords to a diverse set of users. In this context, implementing CC in a network serving $K$ users, each possessing sufficient memory to store a fraction $\gamma$ of the entire library, enables the so-called \emph{global coded caching gain} of $K\gamma+1$. Notably, this delivery speed-up factor can also be aggregated with the spatial multiplexing gain and enhanced to $K\gamma+L$ in a multi-input multi-output (MISO) setup with $L$ antennas at the transmitter~\cite{shariatpanahi2016multi,shariatpanahi2018physical}.
    
% The critical role of multi-antenna connectivity in resolving the practical bottlenecks of CC models has been explored in various studies. For instance, the authors in~\cite{lampiris2018adding} demonstrated that the MISO CC systems are capable of addressing the subpacketization complexity via the integration of signal-level decoding strategies, where the unwanted terms are reconstructed from the local cache memory and removed before the received signal is decoded at the receiver. Later, the proposed idea in \cite{lampiris2018adding} was systematically extended by \cite{salehi2020lowcomplexity} and \cite{parrinello2019fundamental} to \emph{cyclic coded caching} and \emph{shared caching}, respectively, to overcome the subpacketization impediment in MISO CC setups. Accordingly, \cite{10206827} showed that employing the shared-cache model and equipping the transmitter with $L$ transmit antennas can effectively handle the CC configurations with the dynamic user population. The capability of MISO CC schemes to deal with location-dependant applications was studied in~\cite{mahmoodi2021non}, and several works, including~\cite{tolli2017multi,8374074,9923619,10325409}, illustrated the enhancement in rate performance for MISO systems through the implementation of CC under finite signal-to-noise ratio (SNR) conditions.


%The MISO CC works mentioned earlier share a common feature—they all operate with a server connected to a central data library. However, this characteristic limits their applicability in scenarios, such as wireless sensor networks~\cite{9463425,XU2004945}. In these scenarios, users rely on receiving real-time or time-sensitive data, for example, consisting of weather updates, health status, emergency alerts, or online auction details. Since the server lacks a priori knowledge of this information, we can deliver the necessary data to users through two different mechanisms: \textit{1) } Device-to-Device (D2D) caching systems: each user/sensor transmits a part of its measured/cached data directly to the other users~\cite{7342961}, and \textit{2) }~centralized caching systems: each user/sensor sends a part of its measured/cached data to a central server~\cite{8051074}. Subsequently, the server completes the required data processing and transmits the demanded information back to the users. In many applications, e.g., image recognition, the D2D caching systems are not a suitable method to deliver the data, as the size of the data is significantly large, and users are not able to run complex processing on data~\cite{269490}. In this paper, we focus on data delivery and information retrieval in a centralized caching system. Although the information retrieval problem has been studied in various cache-aided single-antenna models, such as coded data shuffling~\cite{8957508,8955811,8754795}, coded distributed computing~\cite{8051074,7935426,8744394}, private coded caching~\cite{9249022}, and cache-aided linear function retrieval~\cite{9378566,9681716}, a centralized CC scheme that enables the data recovery in a cache-aided MISO setup is still missing in the literature.

In this paper, we present a data delivery algorithm for information retrieval in a cache-aided MISO setup, in which a base station (BS) with $L$ transmit antennas serves $K$ single-antenna users, each equipped with the cache ratio of $\gamma$. The BS does not have access to the library, and each user is able to recover its requested data after two phases: \textit{i) } content placement phase, and \textit{ii)} content delivery phase. During the content placement phase, a $\gamma$ portion of the entire library is stored in the cache memory of each user. The content delivery phase commences once the set of active users reveals their required files to the base station (BS), i.e., the central server, and involves two consecutive steps: \textit{1)} Uplink (UL) step, and \textit{2)} Downlink (DL) step. In the uplink step, a set of users transmit their cached data to the BS, and in the DL step, the BS decodes/amplifies its received signals and forwards them to the users. In order to achieve the optimal memory-load tradeoff in the DL, the BS follows a similar approach as in~\cite{shariatpanahi2016multi,shariatpanahi2018physical}, and each user adopts the signal-level decoding method to retrieve its requested file~\cite{lampiris2018adding}. To facilitate the data transmission to the BS during the UL step, we start by considering two naive transmission strategies -- one utilizing only the available spatial multiplexing gain and the other leveraging solely the... global coded caching gain. However, it is observed that neither of these strategies can achieve an UL load equivalent to that of the DL. Accordingly, we devise an UL transmission strategy in which, during each transmission, $K\gamma+L$ users are selected to transmit a clever combination of their cached data to the BS, enabling BS to create all codewords of size $K\gamma+1$. It is proven that this scheme achieves the UL load equal to the optimal DL load, as it benefits from both global coded caching gain and spatial multiplexing gain.

==> MyCommands_old.tex <==
\newtheorem{thm}{Theorem}
\newtheorem{lem}{Lemma}%[section]
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}{Corollary}
\newtheorem{conj}{Conjecture}[section]
\newtheorem{exmp}{Example}%[section]
\theoremstyle{definition}
\newtheorem{defn}{Definition}%[section]
\newtheorem{rem}{Remark}

% Calligraphic Letters
\newcommand{\CA}[0]{{\mathcal{A}}}
\newcommand{\CB}[0]{{\mathcal{B}}}
\newcommand{\CC}[0]{{\mathcal{C}}}
\newcommand{\CD}[0]{{\mathcal{D}}}
\newcommand{\CE}[0]{{\mathcal{E}}}
\newcommand{\CF}[0]{{\mathcal{F}}}
\newcommand{\CG}[0]{{\mathcal{G}}}
\newcommand{\CH}[0]{{\mathcal{H}}}
\newcommand{\CI}[0]{{\mathcal{I}}}
\newcommand{\CJ}[0]{{\mathcal{J}}}
\newcommand{\CK}[0]{{\mathcal{K}}}
\newcommand{\CL}[0]{{\mathcal{L}}}
\newcommand{\CM}[0]{{\mathcal{M}}}
\newcommand{\CN}[0]{{\mathcal{N}}}
\newcommand{\CO}[0]{{\mathcal{O}}}
\newcommand{\CP}[0]{{\mathcal{P}}}
\newcommand{\CQ}[0]{{\mathcal{Q}}}
\newcommand{\CR}[0]{{\mathcal{R}}}
\newcommand{\CS}[0]{{\mathcal{S}}}
\newcommand{\CT}[0]{{\mathcal{T}}}
\newcommand{\CU}[0]{{\mathcal{U}}}
\newcommand{\CV}[0]{{\mathcal{V}}}
\newcommand{\CW}[0]{{\mathcal{W}}}
\newcommand{\CX}[0]{{\mathcal{X}}}
\newcommand{\CY}[0]{{\mathcal{Y}}}
\newcommand{\CZ}[0]{{\mathcal{Z}}}

% Boldface Letters
\newcommand{\Ba}[0]{{\mathbf{a}}}
\newcommand{\Bb}[0]{{\mathbf{b}}}
\newcommand{\Bc}[0]{{\mathbf{c}}}
\newcommand{\Bd}[0]{{\mathbf{d}}}
\newcommand{\Be}[0]{{\mathbf{e}}}
\newcommand{\Bf}[0]{{\mathbf{f}}}
\newcommand{\Bg}[0]{{\mathbf{g}}}
\newcommand{\Bh}[0]{{\mathbf{h}}}
\newcommand{\Bi}[0]{{\mathbf{i}}}
\newcommand{\Bj}[0]{{\mathbf{j}}}
\newcommand{\Bk}[0]{{\mathbf{k}}}
\newcommand{\Bl}[0]{{\mathbf{l}}}
\newcommand{\Bm}[0]{{\mathbf{m}}}
\newcommand{\Bn}[0]{{\mathbf{n}}}
\newcommand{\Bo}[0]{{\mathbf{o}}}
\newcommand{\Bp}[0]{{\mathbf{p}}}
\newcommand{\Bq}[0]{{\mathbf{q}}}
\newcommand{\Br}[0]{{\mathbf{r}}}
\newcommand{\Bs}[0]{{\mathbf{s}}}
\newcommand{\Bt}[0]{{\mathbf{t}}}
\newcommand{\Bu}[0]{{\mathbf{u}}}
\newcommand{\Bv}[0]{{\mathbf{v}}}
\newcommand{\Bw}[0]{{\mathbf{w}}}
\newcommand{\Bx}[0]{{\mathbf{x}}}
\newcommand{\By}[0]{{\mathbf{y}}}
\newcommand{\Bz}[0]{{\mathbf{z}}}

\newcommand{\BA}[0]{{\mathbf{A}}}
\newcommand{\BB}[0]{{\mathbf{B}}}
\newcommand{\BC}[0]{{\mathbf{C}}}
\newcommand{\BD}[0]{{\mathbf{D}}}
\newcommand{\BE}[0]{{\mathbf{E}}}
\newcommand{\BF}[0]{{\mathbf{F}}}
\newcommand{\BG}[0]{{\mathbf{G}}}
\newcommand{\BH}[0]{{\mathbf{H}}}
\newcommand{\BI}[0]{{\mathbf{I}}}
\newcommand{\BJ}[0]{{\mathbf{J}}}
\newcommand{\BK}[0]{{\mathbf{K}}}
\newcommand{\BL}[0]{{\mathbf{L}}}
\newcommand{\BM}[0]{{\mathbf{M}}}
\newcommand{\BN}[0]{{\mathbf{N}}}
\newcommand{\BO}[0]{{\mathbf{O}}}
\newcommand{\BP}[0]{{\mathbf{P}}}
\newcommand{\BQ}[0]{{\mathbf{Q}}}
\newcommand{\BR}[0]{{\mathbf{R}}}
\newcommand{\BS}[0]{{\mathbf{S}}}
\newcommand{\BT}[0]{{\mathbf{T}}}
\newcommand{\BU}[0]{{\mathbf{U}}}
\newcommand{\BV}[0]{{\mathbf{V}}}
\newcommand{\BW}[0]{{\mathbf{W}}}
\newcommand{\BX}[0]{{\mathbf{X}}}
\newcommand{\BY}[0]{{\mathbf{Y}}}
\newcommand{\BZ}[0]{{\mathbf{Z}}}

% Bar over the letters
\newcommand{\Bra}[0]{{\Bar{a}}}
\newcommand{\Brb}[0]{{\Bar{b}}}
\newcommand{\Brc}[0]{{\Bar{c}}}
\newcommand{\Brd}[0]{{\Bar{d}}}
\newcommand{\Bre}[0]{{\Bar{e}}}
\newcommand{\Brf}[0]{{\Bar{f}}}
\newcommand{\Brg}[0]{{\Bar{g}}}
\newcommand{\Brh}[0]{{\Bar{h}}}
\newcommand{\Bri}[0]{{\Bar{i}}}
\newcommand{\Brj}[0]{{\Bar{j}}}
\newcommand{\Brk}[0]{{\Bar{k}}}
\newcommand{\Brl}[0]{{\Bar{l}}}
\newcommand{\Brm}[0]{{\Bar{m}}}
\newcommand{\Brn}[0]{{\Bar{n}}}
\newcommand{\Bro}[0]{{\Bar{o}}}
\newcommand{\Brp}[0]{{\Bar{p}}}
\newcommand{\Brq}[0]{{\Bar{q}}}
\newcommand{\Brr}[0]{{\Bar{r}}}
\newcommand{\Brs}[0]{{\Bar{s}}}
\newcommand{\Brt}[0]{{\Bar{t}}}
\newcommand{\Bru}[0]{{\Bar{u}}}
\newcommand{\Brv}[0]{{\Bar{v}}}
\newcommand{\Brw}[0]{{\Bar{w}}}
\newcommand{\Brx}[0]{{\Bar{x}}}
\newcommand{\Bry}[0]{{\Bar{y}}}
\newcommand{\Brz}[0]{{\Bar{z}}}

\newcommand{\BrA}[0]{{\Bar{A}}}
\newcommand{\BrB}[0]{{\Bar{B}}}
\newcommand{\BrC}[0]{{\Bar{C}}}
\newcommand{\BrD}[0]{{\Bar{D}}}
\newcommand{\BrE}[0]{{\Bar{E}}}
\newcommand{\BrF}[0]{{\Bar{F}}}
\newcommand{\BrG}[0]{{\Bar{G}}}
\newcommand{\BrH}[0]{{\Bar{H}}}
\newcommand{\BrI}[0]{{\Bar{I}}}
\newcommand{\BrJ}[0]{{\Bar{J}}}
\newcommand{\BrK}[0]{{\Bar{K}}}
\newcommand{\BrL}[0]{{\Bar{L}}}
\newcommand{\BrM}[0]{{\Bar{M}}}
\newcommand{\BrN}[0]{{\Bar{N}}}
\newcommand{\BrO}[0]{{\Bar{O}}}
\newcommand{\BrP}[0]{{\Bar{P}}}
\newcommand{\BrQ}[0]{{\Bar{Q}}}
\newcommand{\BrR}[0]{{\Bar{R}}}
\newcommand{\BrS}[0]{{\Bar{S}}}
\newcommand{\BrT}[0]{{\Bar{T}}}
\newcommand{\BrU}[0]{{\Bar{U}}}
\newcommand{\BrV}[0]{{\Bar{V}}}
\newcommand{\BrW}[0]{{\Bar{W}}}
\newcommand{\BrX}[0]{{\Bar{X}}}
\newcommand{\BrY}[0]{{\Bar{Y}}}
\newcommand{\BrZ}[0]{{\Bar{Z}}}

% Serif Letters
\newcommand{\Sfa}[0]{{\mathsf{a}}}
\newcommand{\Sfb}[0]{{\mathsf{b}}}
\newcommand{\Sfc}[0]{{\mathsf{c}}}
\newcommand{\Sfd}[0]{{\mathsf{d}}}
\newcommand{\Sfe}[0]{{\mathsf{e}}}
\newcommand{\Sff}[0]{{\mathsf{f}}}
\newcommand{\Sfg}[0]{{\mathsf{g}}}
\newcommand{\Sfh}[0]{{\mathsf{h}}}
\newcommand{\Sfi}[0]{{\mathsf{i}}}
\newcommand{\Sfj}[0]{{\mathsf{j}}}
\newcommand{\Sfk}[0]{{\mathsf{k}}}
\newcommand{\Sfl}[0]{{\mathsf{l}}}
\newcommand{\Sfm}[0]{{\mathsf{m}}}
\newcommand{\Sfn}[0]{{\mathsf{n}}}
\newcommand{\Sfo}[0]{{\mathsf{o}}}
\newcommand{\Sfp}[0]{{\mathsf{p}}}
\newcommand{\Sfq}[0]{{\mathsf{q}}}
\newcommand{\Sfr}[0]{{\mathsf{r}}}
\newcommand{\Sfs}[0]{{\mathsf{s}}}
\newcommand{\Sft}[0]{{\mathsf{t}}}
\newcommand{\Sfu}[0]{{\mathsf{u}}}
\newcommand{\Sfv}[0]{{\mathsf{v}}}
\newcommand{\Sfw}[0]{{\mathsf{w}}}
\newcommand{\Sfx}[0]{{\mathsf{x}}}
\newcommand{\Sfy}[0]{{\mathsf{y}}}
\newcommand{\Sfz}[0]{{\mathsf{z}}}

\newcommand{\SfA}[0]{{\mathsf{A}}}
\newcommand{\SfB}[0]{{\mathsf{B}}}
\newcommand{\SfC}[0]{{\mathsf{C}}}
\newcommand{\SfD}[0]{{\mathsf{D}}}
\newcommand{\SfE}[0]{{\mathsf{E}}}
\newcommand{\SfF}[0]{{\mathsf{F}}}
\newcommand{\SfG}[0]{{\mathsf{G}}}
\newcommand{\SfH}[0]{{\mathsf{H}}}
\newcommand{\SfI}[0]{{\mathsf{I}}}
\newcommand{\SfJ}[0]{{\mathsf{J}}}
\newcommand{\SfK}[0]{{\mathsf{K}}}
\newcommand{\SfL}[0]{{\mathsf{L}}}
\newcommand{\SfM}[0]{{\mathsf{M}}}
\newcommand{\SfN}[0]{{\mathsf{N}}}
\newcommand{\SfO}[0]{{\mathsf{O}}}
\newcommand{\SfP}[0]{{\mathsf{P}}}
\newcommand{\SfQ}[0]{{\mathsf{Q}}}
\newcommand{\SfR}[0]{{\mathsf{R}}}
\newcommand{\SfS}[0]{{\mathsf{S}}}
\newcommand{\SfT}[0]{{\mathsf{T}}}
\newcommand{\SfU}[0]{{\mathsf{U}}}
\newcommand{\SfV}[0]{{\mathsf{V}}}
\newcommand{\SfW}[0]{{\mathsf{W}}}
\newcommand{\SfX}[0]{{\mathsf{X}}}
\newcommand{\SfY}[0]{{\mathsf{Y}}}
\newcommand{\SfZ}[0]{{\mathsf{Z}}}

%=====================================================================================================================================
% ===========================================================================
% File Name: commands.tex
% File Creation Date: 15.6.1995
% Author: Markku Juntti
% Description: Includes useful commands for Latex edition.
% ===========================================================================

\renewcommand{\Re}{\mbox{Re}}
\renewcommand{\Im}{\mbox{Im}}

% Bold-face Greek letters
\renewcommand{\vec}[1]{\bf{#1}}     %equation styles %vector/matrix

% Figure-specific commands
%\newcommand{\MyRect}[2]{}
\newcommand{\FillGray}[3]{\filldraw[gray!50](#3-1+0.1,#1-#2+0.1) rectangle (#3-0.1,#1-#2+1-0.1)}
\newcommand{\FillBlack}[3]{\filldraw[black!70](#3-1+0.1,#1-#2+0.1) rectangle (#3-0.1,#1-#2+1-0.1)}
\newcommand{\FillHatch}[3]{\fill[pattern=crosshatch, pattern color=black!65](#3-1,#1-#2)rectangle(#3,#1-#2+1)}
\ExplSyntaxOn

\NewDocumentCommand \vect { s o m }
 {
  \IfBooleanTF {#1}
   { \vectaux*{#3} }
   { \IfValueTF {#2} { \vectaux[#2]{#3} } { \vectaux{#3} } }
 }
\DeclarePairedDelimiterX \vectaux [1] {\lbrack} {\rbrack}
 { \, \dbacc_vect:n { #1 } \, }
\cs_new_protected:Npn \dbacc_vect:n #1
 {
  \seq_set_split:Nnn \l_tmpa_seq { , } { #1 }
  \seq_use:Nn \l_tmpa_seq { \enspace }
 }
\ExplSyntaxOff

